Revisiting Huffman Coding: Toward Extreme Performance on Modern GPU Architectures

Today's high-performance computing (HPC) applications are producing vast volumes of data, which are challenging to store and transfer efficiently during the execution, such that data compression is becoming a critical technique to mitigate the storage burden and data movement cost. Huffman coding is arguably the most efficient Entropy coding algorithm in information theory, such that it could be found as a fundamental step in many modern compression algorithms such as DEFLATE. On the other hand, today's HPC applications are more and more relying on the accelerators such as GPU on supercomputers, while Huffman encoding suffers from low throughput on GPUs, resulting in a significant bottleneck in the entire data processing. In this paper, we propose and implement an efficient Huffman encoding approach based on modern GPU architectures, which addresses two key challenges: (1) how to parallelize the entire Huffman encoding algorithm, including codebook construction, and (2) how to fully utilize the high memory-bandwidth feature of modern GPU architectures. The detailed contribution is four-fold. (1) We develop an efficient parallel codebook construction on GPUs that scales effectively with the number of input symbols. (2) We propose a novel reduction based encoding scheme that can efficiently merge the codewords on GPUs. (3) We optimize the overall GPU performance by leveraging the state-of-the-art CUDA APIs such as Cooperative Groups. (4) We evaluate our Huffman encoder thoroughly using six real-world application datasets on two advanced GPUs and compare with our implemented multi-threaded Huffman encoder. Experiments show that our solution can improve the encoding throughput by up to 5.0X and 6.8X on NVIDIA RTX 5000 and V100, respectively, over the state-of-the-art GPU Huffman encoder, and by up to 3.3X over the multi-thread encoder on two 28-core Xeon Platinum 8280 CPUs.

==> listing2/200808_128zone_shared.tex <==
\newcommand\DrawAxis{%
	\draw[very thin] (0, 0) -- (16*\unit, 0);
	% \draw[very thin, gray, densely dotted] (32*\unit, 0) -- (64*\unit, 0);
	\foreach \i in {0,...,16}  { \draw[very thin]       (\i*\unit, -.05) -- (\i*\unit, .05); }
	% \foreach \i in {33,...,64} { \draw[very thin, gray] (\i*\unit, -.05) -- (\i*\unit, .05); }
}

\newcommand\strideone[1]{
	\sffamily
	\bgroup
	\begin{tikzpicture}[y=-1cm]
		\def\bit{.01}
		\def\unit{.32}  %% float32

		\DrawAxis

		\foreach \iter in {1,...,5}
			{
				\pgfmathtruncatemacro{\dist}{2^(\iter-1)};
				\pgfmathtruncatemacro{\bw}{#1*2^(\iter-1)};
				\pgfmathtruncatemacro{\end}{2^(5-\iter)-1};
				\node at (-.3, -1.2-\iter*.1in){\scriptsize\sffamily\iter};
				\foreach \i in {0,...,\end}  {
						\pgfmathparse{int(mod(\i,2))}
						\ifnum0=\pgfmathresult\relax {
								\draw[draw=none, fill=black] (\dist*\i*\unit, .05-\iter*.1in) rectangle ++(\bw*\bit, .35*\unit);
							}
							\else {
								\draw[draw=none, fill=Y] (\dist*\i*\unit, .05-\iter*.1in) rectangle ++(\bw*\bit, .35*\unit);
								% \draw[latex-] (\dist*\i*\unit, .05-\iter*.1in) -- ++(\bw*\bit, 0);
								% \draw[latex-] (\bw*\bit, .05-\iter*.1in) -- ++((\dist*\i*\unit-\bw*\bit), 0);
							}
						\fi
					}

			}
		\begin{scope}[yshift=-.65in]
			\node [fill=black, minimum width=.2in, inner sep=1.5pt, font=\color{white}] (l) at (2.5, 0) {\scriptsize\bfseries L};
			\node [fill=Y,     minimum width=.2in, inner sep=1.5pt] 					(r) at (4.8, 0) {\scriptsize\bfseries R};
			\draw[latex-] (l) to[above, midway] node[yshift=-.5ex] {\scriptsize\itshape concatenate} (r);
		\end{scope}
		% \node {};
	\end{tikzpicture}
	\egroup
}


==> setting/_metadata.tex <==

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%\begin{CCSXML}
%<ccs2012>
%   <concept>
%       <concept_id>10003752.10003809.10010170.10010174</concept_id>
%       <concept_desc>Theory of computation~Massively parallel algorithms</concept_desc>
%       <concept_significance>500</concept_significance>
%       </concept>
% </ccs2012>
%\end{CCSXML}

%\ccsdesc[500]{Theory of computation~Massively parallel algorithms}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.

%\keywords{GPU, Massively Parallel, Lossy Compression}

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

==> setting/acm_template_setting.tex <==

%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
% \setcopyright{acmcopyright}
% \copyrightyear{2018}
% \acmYear{2018}
% \acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
% \acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
% \acmConference[ICS '20]{PPoPP '21: ACM International Conference on Supercomputing}{June 29--July 02, 2020}{Barcelona, Spain}
\acmConference[PPoPP '21]{Principles and Practice of Parallel Programming}{February 27--March 3, 2021}{Seoul, South Korea}
% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection, June 03--05, 2018, Woodstock, NY}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

%%
%% end of the preamble, start of the body of the document source.


%% \title moved to text
%% \title[short title]{full title}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.


\author{Jiannan Tian}
\affiliation{%
	\institution{Washington State University}
	\city{Pullman}\state{WA}\country{USA}
}
\email{jiannan.tian@wsu.edu}


\author{Cody Rivera}
\affiliation{%
	\institution{The University of Alabama}
	\city{Tuscaloosa}\state{AL}\country{USA}
}
\email{cjrivera1@crimson.ua.edu}


\author{Jieyang Chen}
\affiliation{%
	\institution{Oak Ridge National Laboratory}
	\city{Oak Ridge}\state{TN}\country{USA}
}
\email{chenj3@ornl.gov}


\author{Sheng Di}
\affiliation{%
	\institution{Argonne National Laboratory}
	\city{Lemont}\state{IL}\country{USA}
}
\email{sdi1@anl.gov}


\author{Dingwen Tao}
\authornote{Corresponding author: Dingwen Tao, School of EECS, Washington State University, Pullman, WA 99164, USA.}
\affiliation{%
	\institution{Washington State University}
	\city{Pullman}\state{WA}\country{USA}
}
\email{dingwen.tao@wsu.edu}


\author{Franck Cappello}
\affiliation{%
	\institution{Argonne National Laboratory}
	\city{Lemont}\state{IL}\country{USA}
}
\email{cappello@mcs.anl.gov}

\renewcommand{\shortauthors}{Tian et~al.}

\settopmatter{printacmref=false}
\setcopyright{none}
\renewcommand\footnotetextcopyrightpermission[1]{}
\pagestyle{plain}

==> tikz2/_tikz_preamble_nodocclass.tex <==

\usepackage[utf8]{inputenc}

\usepackage{textcomp} 
\usepackage{textgreek}

\usepackage[usenames]{color} 

%used for font color
\usepackage{amssymb, amsmath, bm} 
%\usepackage{sfmath}

%useful to type directly diacritic characters
\usepackage{tikz} 
\usetikzlibrary{shadings} 
\usetikzlibrary{positioning}
\usetikzlibrary{graphs}
\usepackage{booktabs}

% \usepackage[margin=.75in, bottom=1in]{geometry}
\usepackage{lipsum}

\usepackage{xcolor}

\usetikzlibrary{shadows.blur}

\definecolor{RED}{HTML}{d7003a} 
\definecolor{BLUE}{HTML}{003399}
\definecolor{BLUE2}{HTML}{2B66D3}
\definecolor{INK}{HTML}{595857}
\definecolor{YELLOW}{HTML}{f1c40f}
\definecolor{GREEN}{rgb}{0,0.6,0}
\definecolor{MIDGRAY}{rgb}{0.5,0.5,0.5}
\definecolor{MAUVE}{rgb}{0.58,0,0.82}

\usepackage{graphicx} 
\usepackage{libertine}


